Variational Bi-LSTMs

Recurrent neural networks like long short-term memory (LSTM) are important architectures for sequential prediction tasks. LSTMs (and RNNs in general) model sequences along the forward time direction. Bidirectional LSTMs (Bi-LSTMs) on the other hand model sequences along both forward and backward directions and are generally known to perform better at such tasks because they capture a richer representation of the data. In the training of Bi-LSTMs, the forward and backward paths are learned independently. We propose a variant of the Bi-LSTM architecture, which we call Variational Bi-LSTM, that creates a channel between the two paths (during training, but which may be omitted during inference); thus optimizing the two paths jointly. We arrive at this joint objective for our model by minimizing a variational lower bound of the joint likelihood of the data sequence. Our model acts as a regularizer and encourages the two networks to inform each other in making their respective predictions using distinct information. We perform ablation studies to better understand the different components of our model and evaluate the method on various benchmarks, showing state-of-the-art performance.

==> figs/Note.tex <==
Priority experiments:
1. Try activity regularization instead of reconstruction. If activity regularization doesn't work, this analysis becomes an ablation study. If not, then we replace h reconstruction with activity regularization and make it default in our model.

Ablation studies:
1. On datasets where we don't need encoder
a. We train model with encoder and show that KL is small.
b. We find that using the prior mean value of z (from b_tilde) during inference, which shows the model is learning a bias based on backward LSTM for the forward path.
c. Using prior's mean value of z instead of sampling, during training leads to bad results. This shows sampling z during training acts as a regularizer.

2. On datasets where we need encoder:
a. We show KL is large.
b. We find that using the prior mean value of z (from b_tilde) during inference, which shows the model is learning a bias based on backward LSTM for the forward path.
c. Using prior's mean value of z instead of sampling, during training leads to bad results. This shows sampling z during training acts as a regularizer.


-> Ask Alesandro if they have twin network results on PTB.

-> Record ??

Datasets that need encoder:
1. TIMID and Blizzard-- helps and KL is large, so it makes sense
2. IMDB-- KL is large but overfits. Add noise to inputs of encoder and see if it removes overfitting.

Datasets that don't need encoder:
1. PTB-- which makes sense because PTB doesn't have structure.



